Even the Easiest(?) Graph Coloring Problem is not Easy in Streaming!

We study a graph coloring problem that is otherwise easy but becomes quite non-trivial in the one-pass streaming model. In contrast to previous graph coloring problems in streaming that try to find an assignment of colors to vertices, our main work is on estimating the number of conflicting or monochromatic edges given a coloring function that is streaming along with the graph; we call the problem {\sc Conflict-Est}. The coloring function on a vertex can be read or accessed only when the vertex is revealed in the stream. If we need the color on a vertex that has streamed past, then that color, along with its vertex, has to be stored explicitly. We provide algorithms for a graph that is streaming in different variants of the one-pass vertex arrival streaming model, viz. the {\sc Vertex Arrival} ({\sc VA}), {Vertex Arrival With Degree Oracle} ({\sc VAdeg}), {\sc Vertex Arrival in Random Order} ({\sc VArand}) models, with special focus on the random order model. We also provide matching lower bounds for most of the cases. The mainstay of our work is in showing that the properties of a random order stream can be exploited to design streaming algorithms for estimating the number of conflicting edges. We have also obtained a lower bound, though not matching the upper bound, for the random order model. Among all the three models vis-a-vis this problem, we can show a clear separation of power in favor of the {\sc VArand} model.

==> color-lower.tex <==
\section{Lower bounds for \colorverify} \label{sec:sep-valb}

We show a tight lower bound of $\Omega(\frac{1}{\epsilon})$ for the \colorverify problem in the vertex arrival model with degree oracle. For the \colorverify problem in the vertex arrival model we show a tight lower bound of $\Omega(\frac{|V|}{\sqrt |E|})$. These bounds are proved using reductions from the \emph{INDEX} problem in the one-way communication complexity model to the \colorverify problem in graphs in the vertex arrival model. In the INDEX problem, Alice gets an $M$-bit string $X\in \{0,1\}^M$ and Bob gets an integer $j\in [M]$. Both Alice and Bob are unaware of each other's input. Alice can send a message to Bob and Bob has to output $X_j$. It is well known that the lower bound on the message length for the INDEX problem in the one-way communication complexity model is $\Omega(M)$ (See Lemma~\ref{index} in Appendix~\ref{sec:comm}).

\subsection{Lower bound for \colorverify in \vadeg model} \label{sec:sep-vadglbsc}

\begin{theorem}\label{theo:sep-vadglbth}
The lower bound for the \colorverify problem in the \vadeg streaming model is $\Omega(\frac{1}{\vareps})$.
\end{theorem}

\begin{proof}
%To determine the lower bound, we consider a reduction from the INDEX problem in the one-way communication protocol to the \colorverify problem in graphs in the \va model with the degree oracle. 

We show the lower bound using a reduction from the INDEX problem in one-way communication complexity to the \colorverify problem in graphs in the vertex arrival model with access to degree oracle. The reduction works as follows: For each input bit $X_i$, Alice constructs a bipartite graph with bipartition $(L_i,R_i)$, where $L_i$ and $R_i$ are independent sets of size $k$. For any two sets $L_s$ and $R_t$, Alice does not add any edge between vertices in $L_s$ and $R_t$. If $X_i$ equals $1$, then vertices in $L_i$ are colored with color $C_1$, else they are colored with color $C_0$. At the end of the stream, Alice sends this memory state to Bob. Bob colors all vertices in $R_i$ for $1\leq i\neq j \leq M$ with color $C_2$. Vertices in $R_j$ are colored with $C_1$. Moreover, for any index $i\in [M]$, Bob adds all edges between $L_i$ and $R_i$. Access to a degree oracle does not provide any advantage to any protocol on this instance. The only difference is in the construction of the graph.
Now, if $X_j=0$, then there are no monochromatic edges in the graph. However, if $X_j=1$, there are $k^2$ monochromatic edges. The number of vertices in the graph is $n=Mk$ and the number of edges is $m=Mk^2$. The number of conflicting edges in the graph is $k^{2}= \vareps m=\vareps Mk^{2}$.
Therefore, for $M=\frac{1}{\eps}$, distinguishing whether the graph is properly-colored (valid) or at least $\eps$-fraction of edges are monochromatic ($\eps$-far from being valid) requires $\Omega(\frac{1}{\eps})$ space.

%Alice has a $M$-bit input string $X \in \{0,1\}^{M}$ and Bob has an integer $j \in [M]$. The lower bound for space complexity to solve the INDEX problem in the one-way communication model is $\Omega(M)$ [Lemma~\ref{index}]. We consider the stream of vertices $X_{1}, X_{2}, ..., X_{M}$ arriving in an arbitrary order as the input to Alice. For each $X_{i}$, we associate a bipartite graph gadget with it. Each partition consists of k vertices and we denote the left and right partitions as $L_{i}$ and $R_{i}$ respectively. $L_{i}$ and $R_{i}$, $\forall i \in [M]$, are independent sets. When Alice receives the bit $X_{i}$, she colors the vertices of $L_{i}$ with the color $C_{0}$, if $X_{i} = 0$, else, she colors the vertices of $L_{i}$ with the color $C_{1}$, if $X_{i} = 1$. Alice saves this memory state and sends it to Bob. Bob colors all the vertices of  $R_{i}$ with the color $C_{2}$, $\forall i \in [M]$, $i \neq j$. However, for the index $j$, he colors all the vertices of $R_{j}$ with color $C_{1}$.  $\forall i \in [M]$, Bob adds all the edges to the gadget for $X_{i}$ to make it a complete bipartite graph. If $X_{j} = 0$, then the color of $L_{j}$ is $C_{0}$ and there are no conflicting edges, whereas if $X_{j} = 1$, then the color of $L_{j}$ is $C_{1}$ and there will be $k^{2}$ conflicting edges. The number of vertices in the graph, $n$, is $\Theta(Mk)$ while the number of edges in the graph, $m$, is $\Theta(Mk^{2})$ and the number of conflicts in the graph is $k^{2}$.
%\[ k^{2} =  \vareps m = \vareps Mk^{2} \] \[ M = \Omega(\frac{1}{\vareps}) \]
\end{proof}

\subsection{Lower bound for \colorverify in \va model} \label{sec:sep-vaaolbsc}

\begin{theorem}\label{theo:sep-vaaolbth} The space lower bound for the \colorverify problem in the \va model is $\Omega\left(\frac{|V|}{\sqrt{|E|}}\right)$. \end{theorem}

\begin{proof} We show the lower bound using a reduction from the INDEX problem in one-way communication complexity to the \colorverify problem in graphs in the order vertex arrival model. For each input bit $X_i$, Alice constructs a bipartite graph with bipartition $(L_i,R_i)$, where $L_i$ and $R_i$ are independent sets of size $k$. For any two sets $L_s$ and $R_t$, Alice does not add any edge between vertices in $L_s$ and $R_t$. If $X_i$ equals $1$, then vertices in $L_i$ are colored with color $C_1$, else they are colored with color $C_0$. At the end of the stream, Alice sends this memory state to Bob. Bob colors all vertices in $R_i$ for $1\leq i\leq M$ with color $C_1$. Moreover, for index $j$, he adds all the edges between $L_j$ and $R_j$ to make it a complete bipartite graph. Now, if $X_j=0$, then there are no monochromatic edges. However, if $X_j=1$, there are $k^2$ monochromatic edges. We have the number of vertices in the graph $n=Mk$ and the number of edges $m=k^2$. Therefore, for $M=\frac{n}{\sqrt{m}}$ or $\frac{|V|}{\sqrt{|E|}}$, distinguishing whether the graph is properly-colored (valid) or all of its edges are monochromatic ($\eps$-far from being valid) requires $\Omega\left(\frac{|V|}{\sqrt{|E|}}\right)$ space.


%To determine the lower bound, we consider a reduction from the INDEX problem in the one-way communication protocol to the \colorverify problem in graphs in the arbitrary order \va model.

%Alice has a $M$-bit input string $X \in \{0,1\}^{M}$ and Bob has an integer $j \in [M]$. The lower bound for space complexity to solve the INDEX problem in the one-way communication model is $\Omega(M)$ [Lemma~\ref{index}]. 
%We consider the stream of vertices $X_{1}, X_{2}, ..., X_{M}$ arriving in an arbitrary order as the input to Alice. For each $X_{i}$, we associate a bipartite graph gadget with it. Each partition consists of k vertices and we denote the left and right partitions as $L_{i}$ and $R_{i}$ respectively. $L_{i}$ and $R_{i}$, $\forall i \in [M]$, are independent sets. When Alice receives the bit $X_{i}$, she colors the vertices of $L_{i}$ with the color $C_{0}$, if $X_{i} = 0$, else, she colors the vertices of $L_{i}$ with the color $C_{1}$, if $X_{i} = 1$. Alice saves this memory state and sends it to Bob. Bob colors all the vertices of  $R_{i}$ with the color $C_{1}$, $\forall i \in [M]$. However, for the index $j$, he adds all the edges to the gadget for $X_{j}$ to make it a complete bipartite graph. If $X_{j} = 0$, then the color of $L_{j}$ is $C_{0}$ and there are no conflicting edges, whereas if $X_{j} = 1$, then the color of $L_{j}$ is $C_{1}$ and there will be $k^{2}$ conflicting edges. The number of vertices in the graph, $n$, is $\Theta(Mk)$ while the number of edges in the graph, $m$, is $\Theta(k^{2})$. Given $n$ and $m$, we can set the values of $M$ and $k$ accordingly.
%\[ k ={\sqrt m} \] \[ M = \Omega(\frac{n}{\sqrt m}) \]
\end{proof}


